Calibrating Energy-based Generative Adversarial Networks

In this paper, we propose to equip Generative Adversarial Networks with the ability to produce direct energy estimates for samples.Specifically, we propose a flexible adversarial training framework, and prove this framework not only ensures the generator converges to the true data distribution, but also enables the discriminator to retain the density information at the global optimal. We derive the analytic form of the induced solution, and analyze the properties. In order to make the proposed framework trainable in practice, we introduce two effective approximation techniques. Empirically, the experiment results closely match our theoretical analysis, verifying the discriminator is able to recover the energy of data distribution.

==> 4-interpretation.tex <==
\section{Understanding the Effectiveness}
\label{sec:interpretation}

In the previous section, we have shown the proposed formulation allows the discriminator to retain density information within the data support.
Here, we hope to provide a more intuitive understanding of why this formulation provides this advantage over normal GAN and its previous variants.
% At the same time, the provided interpretation also explains the Remark \ref{thm:reverse_regularization}.

To do this, it is convenient to think about the gradient w.r.t. the generator network.
In the case of original GAN, there is only one source of gradient from the discriminator, whose effect is to increase the probability (lower the energy) of generated samples.
Therefore, whenever the discriminator has the information of relative density, its gradient w.r.t. the generator will push the generator to \textit{only} generate samples with the highest density.
As a result, to prevent the generator from collapsing into only generate the highest-probability samples, the discriminator must forget all density information and produce flat energy inside the data support.
The same reasoning directly carries to EBGAN objective without the pull away term, and the case \eqref{eq:constant_objective} where $K(\pg)$ is a constant.

In contrast, in the proposed formulation, the generator receives gradients from two sources, one from the discriminator and another from the regularization term. 
Thus, the gradient from the regularization can be used to balance (cancel out) the gradient from a discriminator with density information at the optimal.
Hence, it allows the optimal discriminator to retrain density information.
However, it is worthy mentioning that simply adding regularization to the generator under the $f$-GAN family formulation will \textit{not} induce an optimal discriminator with density information (see appendix \ref{sec:fgan_appendix}).

In addition to this interpretation, we provide another optimization based explanation of why our proposed formulation works in appendix \ref{sec:additional_interpretation}. 


==> analysis.tex <==
%!TEX root = main.tex
\section{Duality-based Analysis}
	
% motivation
\subsection{Interpretation from the GAN Perspective}
In section \ref{sec:informal_discussion}, we mentioned that by optimizing the objective given by $\mathcal{L}_c$~\eqref{eq:objective_c} and $\mathcal{L}_g$~\eqref{eq:objective_g}, we can reach the \textbf{desired solution} that 
	\begin{equation}
		p_g^* = p_c^* = p_\text{data}
	\end{equation}
	The interpretation follows Taesup's work, rooted in training an energy-based model with negative samples from directed generator.
	
	In this section, we try to connect this interpretation to Scalar-output GAN (or Energy-based GAN paper), and discuss the following findings
	\begin{itemize}
		\item why the entropy term is essential to reaching the desired results, especially compared with the Scalar-output GAN without the entropy term
		\item how the entropy term can be replaced with other terms to result in other reasonable solutions
	\end{itemize}
	In addition, we also provide a interpretation of the optimization process from the perspective of dual-primal sub-gradient method.
	
	% sub-section for concrete analysis
	\subsection{Concrete Analysis}
	\label{sec:concrete_analysis}
	Let's first formulate the problem from a Scalar-output GAN perspective, i.e. a minimax game. 
	For simplicity of the analysis, we only consider the case that data $x$ resides in a data space $\mathcal{X}$ with countably many values.~\footnote{To extend the discussion to the infinite-dimension case (i.e. continuous case), it will require functional analysis techniques.}
	
	The minimax game formulation is as follows
	
	\begin{equation}
		\label{eq:original_problem}
		\max_{C} \min_{p_g \in \mathcal{P}} \sum_{x \in \mathcal{X}} p_g(x) C(x) - \sum_{x \in \mathcal{X}} p_\text{data}(x) C(x) + h(p_g)
	\end{equation}
	where $C$ is the energy function to learn, $\mathcal{P} = \{p \mid \forall x \in \mathcal{X}, p(x) \geq 0,  \sum_{x \in \mathcal{X}} p(x) = 1\}$, and $h(p_g)$ is a convex function of every $p_g(x)$ term, which essentially poses extra regularization on the $p_g$.
	
	Note that \eqref{eq:original_problem} is actually the Lagrange dual problem of the following one
	
	\begin{equation}
		\label{eq:primal_problem}
		\begin{aligned}
			\min_{p_g \in \mathcal{P}}&\quad  h(p_g) \\
			\text{s.t.}&\quad p_g(x) - p_\text{data}(x) = 0, \forall x
		\end{aligned}
	\end{equation}
	where $C(x)$ shows up in \eqref{eq:original_problem} as the dual variable for the equality constraint.
	This duality relationship is initially observed by the \textit{Adversarial Imitation Learning} paper~\footnote{\url{https://arxiv.org/abs/1606.03476}}.
	However, they don't characterize the dual solution $C^*$, and fully focus on $g_p^*$.
	
	Since $\mathcal{P}$ can be explicitly written as a series of convex inequality constraints and affine equality constraints, the primal problem can be rewritten as
	\begin{equation}
		\label{eq:primal_problem_new}
		\begin{aligned}
			\min_{p_g}&\quad  h(p_g) \\
			\text{s.t.}
			&\quad -p_g(x) \leq 0, \forall x \\
			&\quad p_g(x) - p_\text{data}(x) = 0, \forall x \\
			&\quad \sum_{x \in \mathcal{X}} p_g(x) - 1 = 0
		\end{aligned}
	\end{equation}
	
	Based on the new formulation with explicit constraints \eqref{eq:primal_problem_new}, the new Lagrange function is
	\begin{equation}
		\label{eq:lagrange_function}
		L(p_g, \mu, C, \lambda) = h(p_g) - \sum_{x \in \mathcal{X}} \mu(x)p_g(x) + \sum_{x \in \mathcal{X}} C(x) \Big( p_g(x) - p_\text{data}(x) \Big) + \lambda (\sum_{x \in \mathcal{X}} p_g(x) - 1)
	\end{equation}
	where $\mu, C, \lambda$ are the dual variables.
	
	Notice that the problem \eqref{eq:primal_problem_new} is a convex optimization problem with countably many convex inequality constraints and affine equality constraints.
	Therefore, it satisfies the Slater's condition and the strong duality holds. 
	Hence, we can use the KKT conditions to characterize the optimal solutions for both primal and dual variables.
	Specifically, the KKT conditions for $p_g^*, \mu^*, C^*, \lambda^*$ are
	\begin{equation}
		\begin{aligned}
			\nabla_{p_g(x)} h\mid_{p_g^*} + C^*(x) - \mu^*(x) + \lambda^* = 0,& \quad\forall x & \text{(stationarity)} \\
			\mu^*(x) p_g^*(x) = 0^{m},& \quad\forall x & \text{(complement slackness)} \\
			p_g(x) \geq 0, \quad p_g^*(x) = p_\text{data}(x),& \quad\forall x & \text{(primal feasibility)} \\
			\sum_{x \in \mathcal{X}} p_g(x) = 1 && \text{(primal feasibility)} \\
			\mu^*(x) \geq 0,& \quad\forall x & \text{(dual feasibility)}
		\end{aligned}
	\end{equation}
	
	Rearranging the conditions above, we can characterize the energy function $C^*$ at equilibrium as follows
	\begin{equation}
		\begin{aligned}
			C^*(x) &= -\nabla_{p_g(x)} h(p_\text{data}) - \lambda^* + \mu^*(x) \\
			\mu^*(x) &=  
			\begin{cases}
				0, & p_\text{data}(x) > 0 \\
				\R_+, & p_\text{data}(x) = 0
			\end{cases}
		\end{aligned}
	\end{equation}
	where $\R_+$ represents the set of non-negative real numbers.
	
	Now, let's consider special cases of the convex function $h(\cdot)$.
	For easier reference, we refer to the subset $\mathcal{X}_{>} = \{ p_\text{data}(x) > 0\}$ as data area, and its complement $\mathcal{X}_{=} = \{ p_\text{data}(x) = 0\}$ as non-data area. 
	\begin{enumerate}
		% no term case
		\item When $h(p_g) = 0$, i.e. when there is no extra cost, 
		\begin{equation}
			\begin{aligned}
				C_\text{none}^*(x) &=  
				\begin{cases}
					- \lambda^*, & p_\text{data}(x) > 0 \\
					- \lambda^* + \R_+, & p_\text{data}(x) = 0
				\end{cases}
			\end{aligned}
		\end{equation}
		Basically, this means the energy function will be flat in the data area $\mathcal{X}_{>}$. 
		So, it \textbf{cannot distinguish slightly probable area from highly probable area}. 
		
		However, the flat energy in data area is guaranteed to be no larger than ($\leq$) the energy in the non-data area, because $R^*$ indicates a underdetermined non-negative value.
		Therefore, the energy function only has a slight possibility of \textbf{distinguishing data area $\mathcal{X}_{>}$ from non-data area $\mathcal{X}_{=}$}. 
		
		% entropy term case
		\item When $h(p_g) = \sum_{x \in \mathcal{X}} p_g(x) \log p_g(x)$ (i.e. adding the entropy term), we have $\nabla_{p_g(x)} h(p_\text{data}) = \log p_\text{data}(x) + 1$
		\begin{equation}
			\label{eq:entropy_sol}
			\begin{aligned}
				C_\text{ent}^*(x) &= -\log p_\text{data}(x) - 1 - \lambda^* + \mu^*(x) \\
				\mu^*(x) &=  
				\begin{cases}
					0, & p_\text{data}(x) > 0 \\
					\R_+, & p_\text{data}(x) = 0
				\end{cases}
			\end{aligned}
		\end{equation}
		Although this solution is still underdetermined, it has two desirable properties
		\begin{itemize}
			\item the data area always has lower energy compared to non-data area because $\lim_{p_\text{data}(x) \rightarrow 0} C_\text{ent}^*(x) \rightarrow \infty$, which is greater than any finite energy value of $C_\text{ent}^*(x)$ where $p_\text{data}(x) > 0$. 
			
			\item within the data area, the energy function has lower value where the data has higher probability, simply because $-\log(\cdot)$ is monotone decreasing. Thus, the underdetermined dual variable $\lambda^*$ only controls the ``global'' energy baseline.
		\end{itemize}
		Finally, examining the optimal energy function in the data area, it's exactly the negative log probability, which can recover the data distribution by
		\begin{equation}
			\label{eq:undirected_prob_entropy}
			p_\text{data}(x) = \frac{\exp\Big( - \beta \big(C_\text{ent}^*(x) - \mu^*(x)\big) \Big)}{\sum_{x' \in \mathcal{X}} \exp\Big( - \beta \big(C_\text{ent}^*(x') - \mu^*(x')\big) \Big)}
		\end{equation}
		where $\beta$ is the temperature parameter. 
		When plugging equation \eqref{eq:entropy_sol} into equation \eqref{eq:undirected_prob_entropy}, we can see that the underdetermined baseline constant $\lambda^*$ cancel out.
		
		% L2 norm term case
		\item When $h(p_g) = \frac{1}{2} \sum_{x \in \mathcal{X}} p_g(x)^2$, i.e. the $L_2$ norm regularization, we have $\nabla_{p_g(x)} h(p_\text{data}) = p_\text{data}(x)$, and it follows
		\begin{equation}
			\label{eq:l2_sol}
			\begin{aligned}
				C_{L_2}^*(x) &= - p_\text{data}(x) - \lambda^* + \mu^*(x) \\
				\mu^*(x) &=  
				\begin{cases}
					0, & p_\text{data}(x) > 0 \\
					\R_+, & p_\text{data}(x) = 0
				\end{cases}
			\end{aligned}
		\end{equation}
		Compared to the entropy solution \eqref{eq:entropy_sol}, this solution has very similar properties. 
		A difference lies in that the discriminant power of $C^*_{L_2}$ is \textbf{linear} w.r.t. $p_\text{data}(x)$, while the discriminant power of $C^*_\text{ent}$ is \textbf{log-linear} w.r.t. $p_\text{data}(x)$.
		Thus, $C^*_{L_2}$ is less sensitive to extremely low value of $p_\text{data}(x)$, while $C^*_\text{ent}$ is less sensitive to extremely high value of $p_\text{data}(x)$.
		
		In addition, as an advantage of $C^*_{L_2}$ over $C^*_\text{ent}$, to recover $p_\text{data}$, we don't need to compute the partition function anymore. 
		However, the disadvantage is that we have to solve the baseline constant $\lambda^*$ exactly. 
	\end{enumerate}
	
	\subsection{Dual-Primal Sub-gradient Method Interpretation}
	
	Based on the dual analysis given in section \ref{sec:concrete_analysis}, iterative parameter updates based on the gradients of \eqref{eq:objective_c} and \eqref{eq:objective_g} respectively can be seen as one update under dual-primal sub-gradient method.
	For intro-level understanding, please refer to the lecture notes~\footnote{\url{http://stanford.edu/class/ee364b/lectures/primal_dual_subgrad_slides.pdf}}.
	For more detailed understanding, please refer to the paper~\footnote{\url{http://ium.mccme.ru/postscript/s12/GS-Nesterov\%20Primal-dual.pdf}}.
